A-type Supergiant Abundances in the SMC: Probes of Evolution

New abundances of N, O, Na, Mg, Si, Ca, Sc, Ti, Cr, Fe, Sr, Zr, and Ba are presented for 10 A-type supergiants in the SMC, plus upper limits for C. In interpreting the CNO results for constraints on stellar evolution theories, careful attention has been paid to the comparison abundances, i.e., the present day abundances of SMC nebulae and B-dwarf stars. These new results are also compared to published results from F-K supergiant analyses, and found to be in good agreement when both sets of data are carefully examined as differential (SMC minus Galactic standard) abundances. With the exception of nitrogen, very small star-to-star abundance variations are found for all elements in this analysis. The N variations are not predicted by standard stellar evolution models. Instead, the results support the new predictions reported from rotating stellar models, where the range in nitrogen is the result of partial mixing of CN-cycled gas from the stellar interior due to main-sequence rotation at different rates (c.f., Langer & Heger 1998). The overall overabundance of nitrogen in the sampled stars also implies these stars have undergone the first dredge-up in addition to having been mixed while on the main-sequence. The alpha-elements (O, Mg, Si, Ca, Ti) have similar underabundances to Fe, which is not the same as seen in metal-poor stars in the solar neighborhood of the Galaxy. In addition, certain light s-process elements (Zr, Ba) are slightly more underabundant than Fe, which is predicted by the bursting chemical evolution model presented by Pagel & Tautvaisiene (1998) for the SMC.

==> tab1.tex <==
%table 1
\begin{table*}
\caption[]{SMC A-Type Supergiant Parameters }
\begin{flushleft}
\begin{tabular}{lllllccc} 
\noalign{\smallskip}
\tableline
\noalign{\smallskip}
AV & Sk & Sp.Ty & Sp.Ty & V & \teff & \logg &  \underline{Velocities \ (km\,s$^{\rm -1}$)} \\
   &    & OLD   &  NEW  &   &       &       &  $\xi$ \ \ \ \ \ \  v$_{\rm rad}$  \ \ \  $v$sin$i$ \\ 
\noalign{\smallskip}
\tableline
\noalign{\smallskip}
AV 110  & Sk~49  & A0 Ia  & A1 Ia  & 12.1 & 9500 & 1.4 & 4 \ \ \ \ \ +160 \ \ \ \ \ 25 \\
AV 298  &        & A0 Iab & A1 Ia  & 12.5 & 9400 & 1.7 & 3 \ \ \ \ \ +155 \ \ \ \ \ 15 \\
AV 392  & Sk~125 & A3 Ib  & A3 Ib  & 12.5 & 8500 & 1.7 & 3 \ \ \ \ \ +135 \ \ \ \ \ 25 \\
AV 136  & Sk~54  & A0 Ia  & A5 Iab & 11.0 & 8200 & 1.0 & 6 \ \ \ \ \ +160 \ \ \ \ \ 20 \\
AV 463  & Sk~146 & A2 Ib  & A7 Ib  & 12.2 & 8000 & 1.3 & 4 \ \ \ \ \ +170 \ \ \ \ \ 25 \\
AV 478  & Sk~154 & A0 Ib  & A7 Iab & 11.6 & 8100 & 1.1 & 5 \ \ \ \ \ +180 \ \ \ \ \ 15 \\
AV 254  & Sk~89  & A2 Ib  & A7 Iab & 11.6 & 8000 & 1.1 & 6 \ \ \ \ \ +180 \ \ \ \ \ 20 \\
AV 442  & Sk~136 & A3 Iab & A7 Iab & 11.4 & 7900 & 0.9 & 7 \ \ \ \ \ +185 \ \ \ \ \ 20 \\
AV 213  & Sk~75  & A2 Iab & F0 Ia  & 12.0 & 7500 & 0.5 & 6 \ \ \ \ \ +175 \ \ \ \ \ 20 \\
AV 174  & Sk~63  & A7 Iab & F2 Iab & 12.4 & 7200 & 0.8 & 4 \ \ \ \ \ +165 \ \ \ \ \ 35 \\
\noalign{\smallskip}
\tableline
\noalign{\smallskip}
\end{tabular}
\end{flushleft}
\end{table*}




==> tab10.tex <==
%table 9
\begin{table*}
\caption[]{SMC Nebular and B-Star Abundances}
\begin{flushleft}
\begin{tabular}{c|lcll|lcr|c} 
\noalign{\smallskip}
\tableline
\noalign{\smallskip}
Elem &  & Nebulae & &   &  & B-stars   &        & Adopted \\ 
     & D84 & RD90 & G95 & K98 &  GAL & R93 & ( =  )  &  \\
\noalign{\smallskip}
\tableline
\noalign{\smallskip}
C  & 7.2 & ... &  7.4 & \ \ 7.5 & 8.3 & $-$0.9  & ( 7.4)   & 7.4 \\
N  & 6.5 & 6.6 &  6.3 & \ \ 6.6 & 7.8 & $<$-1.1 & ($<$6.7) & 6.6 \\
O  & 8.0 & 8.1 &  8.1 & \ \ 8.1 & 8.6 & $-$0.5  & ( 8.1)   & 8.1 \\
\noalign{\smallskip}
\tableline
\noalign{\smallskip}
\end{tabular} 
\begin{minipage}[t]{18cm}{
D84 = Dufour 1984, RD90 = Russell \& Dopita 1990, G95 = Garnett \etal
1995, K98 = Kurt \etal 1998, R93 = Rolleston \etal 1993.   Note that
the B-stars/nebular C abundance is 0.3~dex less than that reported from
F-K supergiants (see discussion in text).
}
\end{minipage}
\end{flushleft}
\end{table*}


==> tab11.tex <==
%appendix A
\begin{deluxetable}{lllrrlrrrrrrrrrr}
\tablewidth{0pc}
\tablecaption{Line Data and Equivalent Widths}
\tablehead{
\colhead{Elem} & \colhead{Mult} & \colhead{Wavel} & \colhead{$\chi$} & 
\colhead{log~gf} &  \colhead{Comm} & 
\colhead{110} & \colhead{298} & \colhead{392} & \colhead{136} & 
\colhead{463} & \colhead{478} & \colhead{254} & \colhead{442} & 
\colhead{213} & \colhead{174} }
\startdata
 700 &    3 &  7423.63 &  10.33 &  -0.69 & zhu   &  \nodata &  \nodata &  \nodata &   31 &  \nodata &   79 &  \nodata &   58 &   90 &  \nodata \nl
 700 &    3 &  7442.28 &  10.33 &  -0.40 & zhu   &   48 &   57 &  \nodata &   66 &  \nodata &   90 &  \nodata &   64 &  150 &  \nodata \nl
 700 &    3 &  7468.29 &  10.34 &  -0.21 & zhu   &   78 &   65 &  \nodata &  105 &   80 &  134 &   80 &   85 &  \nodata &  \nodata \nl
 700 &    2 &  8210.64 &  10.33 &  -0.68 & zhu   &  \nodata &  \nodata &  \nodata &   58 &  \nodata &   22 &  \nodata &  \nodata &   94 &  \nodata \nl
 700 &    2 &  8216.28 &  10.34 &   0.09 & zhu   &   75 &   96 &  \nodata &  190 &   60 &  175 &  109 &  179 &  \nodata &   54 \nl
 700 &    2 &  8223.07 &  10.33 &  -0.29 & zhu   &  \nodata &  \nodata &  \nodata &  167 &   46 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
 700 &    2 &  8242.34 &  10.34 &  -0.26 & zhu   &   55 &  \nodata &  \nodata &  105 &  \nodata &  116 &  \nodata &   77 &  154 &  \nodata \nl
 800 &   10 &  6155.99 &  10.74 &  -0.67 & op    &   14 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   27 &  \nodata &  \nodata \nl
 800 &   10 &  6156.78 &  10.74 &  -0.45 & op    &   16 &  \nodata &  \nodata &  \nodata &  \nodata &   36 &  \nodata &   32 &  \nodata &  \nodata \nl
 800 &   10 &  6158.19 &  10.74 &  -0.31 & op    &   36 &   36 &  \nodata &   57 &   53 &   40 &   74 &   45 &   38 &  \nodata \nl
 800 &    9 &  6454.48 &  10.74 &  -1.14 & op    &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   17 &  \nodata &  \nodata \nl
1100 &    1 &  5889.95 &   0.00 &   0.11 & wm    &  \nodata &  \nodata &  \nodata &  \nodata &  131 &  125 &  235 &  189 &  \nodata &  \nodata \nl
1100 &    1 &  5895.92 &   0.00 &  -0.19 & wm    &  \nodata &  \nodata &  \nodata &  \nodata &  105 &   93 &  157 &  126 &  \nodata &  \nodata \nl
1100 &    4 &  8194.82 &   2.10 &   0.51 & wm    &  \nodata &  \nodata &   50 &  \nodata &  \nodata &   63 &  \nodata &  \nodata &  156 &  110 \nl
1200 &   11 &  4702.98 &   4.35 &  -0.37 & wm    &  \nodata &   10 &   25 &   20 &   50 &   13 &   24 &   16 &   40 &   97 \nl
1200 &    2 &  5167.32 &   2.71 &  -0.86 & wm    &  \nodata &   13 &   64 &   60 &  130 &   79 &  100 &   88 &  130 &  \nodata \nl
1200 &    2 &  5172.68 &   2.71 &  -0.38 & wm    &   20 &   29 &   97 &   74 &  160 &  118 &  155 &  137 &  \nodata &  \nodata \nl
1200 &    2 &  5183.60 &   2.72 &  -0.16 & wm    &   36 &   46 &  124 &   92 &  202 &  148 &  184 &  180 &  \nodata &  \nodata \nl
1201 &   10 &  4390.59 &  10.00 &  -0.53 & wsm   &  \nodata &   24 &  \nodata &  \nodata &  \nodata &   31 &  \nodata &  \nodata &  \nodata &  \nodata \nl
1201 &    9 &  4427.99 &  10.00 &  -1.21 & wsm   &  \nodata &  \nodata &   11 &  \nodata &   19 &  \nodata &   11 &  \nodata &  \nodata &  \nodata \nl
1201 &    9 &  4433.99 &  10.00 &  -0.91 & wsm   &  \nodata &  \nodata &   15 &  \nodata &   21 &  \nodata &   13 &   21 &   18 &  \nodata \nl
1201 &   19 &  4436.48 &  11.57 &  -0.89 & wsm   &  \nodata &   10 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
1201 &    8 &  7877.13 &  10.00 &   0.39 & wsm   &  \nodata &   51 &   50 &   91 &  \nodata &   38 &  \nodata &   49 &   42 &  \nodata \nl
1201 &    8 &  7896.37 &  10.00 &   0.65 & wsm   &  100 &   90 &  100 &  150 &  142 &  100 &   86 &  102 &  110 &   98 \nl
1401 &    3 &  4128.05 &   9.84 &   0.31 & wm    &  135 &   66 &  \nodata &  \nodata &  \nodata &  103 &  \nodata &  103 &  127 &  \nodata \nl
1401 &    3 &  4130.88 &   9.84 &   0.46 & wm    &  152 &   91 &  \nodata &  145 &   92 &  100 &   93 &  102 &  128 &  \nodata \nl
1401 &    5 &  5041.06 &  10.07 &   0.17 & nk    &  101 &   59 &   65 &  103 &   53 &   59 &   57 &   52 &   55 &  \nodata \nl
1401 &    5 &  5056.02 &  10.08 &   0.59 & nk    &  \nodata &   72 &   82 &  153 &   79 &  103 &   85 &  \nodata &   96 &   69 \nl
1401 &    4 &  5957.61 &  10.07 &  -0.35 & wm    &   47 &  \nodata &  \nodata &   39 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
1401 &    4 &  5978.97 &  10.07 &  -0.06 & wm    &   70 &  \nodata &  \nodata &   62 &  \nodata &  \nodata &  \nodata &   28 &  \nodata &  \nodata \nl
1401 &    2 &  6347.09 &   8.12 &   0.23 & wm    &  \nodata &  146 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
1401 &    2 &  6371.36 &   8.12 &  -0.08 & wm    &  \nodata &  126 &  145 &  \nodata &  \nodata &  \nodata &  204 &  \nodata &  \nodata &  150 \nl
2000 &    2 &  4226.73 &   0.00 &   0.24 & wm    &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   45 &   75 &   59 &  119 &  \nodata \nl
2000 &    4 &  4425.44 &   1.88 &  -0.39 & wm    &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   58 \nl
2000 &    4 &  4435.30 &   1.89 &   0.00 & wm    &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  130 \nl
2000 &    3 &  6162.17 &   1.90 &  -0.09 & wm    &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  116 \nl
2000 &   18 &  6439.07 &   2.53 &   0.47 & wm    &  \nodata &  \nodata &   65 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2000 &   18 &  6462.57 &   2.52 &   0.31 & wm    &  \nodata &  \nodata &  139 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   73 \nl
2000 &   30 &  7148.15 &   2.71 &   0.00 & wm    &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   52 \nl
2001 &   13 &  8203.20 &   7.51 &   0.30 & wsm   &  \nodata &  \nodata &  \nodata &  \nodata &  116 &  \nodata &   39 &   39 &  \nodata &  165 \nl
2001 &   13 &  8250.20 &   7.52 &   0.57 & wsm   &  \nodata &  \nodata &  \nodata &   61 &  142 &   55 &  117 &   76 &  100 &  \nodata \nl
2001 &   13 &  8256.10 &   7.52 &  -0.40 & wsm   &  \nodata &  \nodata &  \nodata &  \nodata &   62 &  \nodata &  \nodata &  \nodata &   42 &   48 \nl
2101 &    8 &  4014.49 &   0.32 &  -1.66 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   15 &   15 &   48 &   89 \nl
2101 &    7 &  4246.83 &   0.32 &   0.32 &  nk   &  \nodata &   18 &   85 &  \nodata &  175 &  142 &  198 &  200: &  \nodata &  \nodata \nl
2101 &   15 &  4305.72 &   0.60 &  -1.21 &  nk   &  \nodata &  \nodata &   17 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2101 &   15 &  4320.75 &   0.61 &  -0.26 &  nk   &  \nodata &  \nodata &   76 &   75 &  \nodata &  119 &  170 &  150 &  \nodata &  \nodata \nl
2101 &   15 &  4325.01 &   0.60 &  -0.44 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   43 &   91 &   73 &  142 &  \nodata \nl
2101 &   14 &  4420.66 &   0.62 &  -2.03 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   19 \nl
2101 &   23 &  5031.02 &   1.36 &  -0.34 &  nk   &  \nodata &  \nodata &  \nodata &   20 &   55 &  \nodata &   50 &   35 &   79 &  119 \nl
2201 &   11 &  4012.37 &   0.57 &  -1.61 &  mfw  &  \nodata &   24 &  105 &  110 &  159 &  \nodata &  178 &  161 &  \nodata &  \nodata \nl
2201 &   11 &  4025.14 &   0.61 &  -1.98 &  mfw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  102 &   82 &  163 &  \nodata \nl
2201 &   87 &  4028.33 &   1.89 &  -1.00 &  mfw  &  \nodata &   18 &   66 &   86 &  122 &  100 &  145 &  130 &  \nodata &  \nodata \nl
2201 &   87 &  4053.81 &   1.89 &  -1.21 &  mfw  &  \nodata &  \nodata &   69 &   92 &  121 &  \nodata &  142 &  122 &  \nodata &  \nodata \nl
2201 &   87 &  4053.83 &   1.89 &  -1.21 &  mfw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   95 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2201 &   21 &  4161.53 &   1.08 &  -2.36 &  mfw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   54 &  \nodata &  55 &  \nodata &  \nodata \nl
2201 &  105 &  4163.60 &   2.59 &  -0.40 &  mfw  &  \nodata &   16 &   96 &  105 &  137 &  121 &  155 &  151 &  \nodata &  \nodata \nl
2201 &  105 &  4171.90 &   2.60 &  -0.56 &  mfw  &  \nodata &   20 &   80 &   97 &  142 &  \nodata &  152 &  139 &  \nodata &  \nodata \nl
2201 &   33 &  4227.34 &   1.13 &  -2.36 &  mfw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   34 &   44 &   42 &   75 &  \nodata \nl
2201 &   20 &  4287.89 &   1.08 &  -2.02 &  mfw  &  \nodata &  \nodata &   60 &   53 &  101 &   68 &   96 &   91 &  145 &  \nodata \nl
2201 &   41 &  4290.22 &   1.16 &  -1.12 &  mfw  &  \nodata &   26 &  120 &  135 &  \nodata &  194 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2201 &   20 &  4294.10 &   1.08 &  -1.11 &  mfw  &  \nodata &   37 &  105 &  130 &  \nodata &  187 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2201 &   41 &  4300.05 &   1.18 &  -0.77 &  mfw  &   30 &   51 &  151 &  170 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2201 &   41 &  4301.93 &   1.16 &  -1.16 &  mfw  &  \nodata &   19 &  \nodata &   91 &  \nodata &  129 &  173 &  159 &  \nodata &  \nodata \nl
2201 &   41 &  4307.90 &   1.16 &  -1.29 &  mfw  &  \nodata &   29 &  111 &  105 &  \nodata &  165 &  203 &  194 &  \nodata &  \nodata \nl
2201 &   41 &  4312.86 &   1.18 &  -1.16 &  mfw  &  \nodata &   27 &   82 &   86 &  161 &  140 &  192 &  178 &  \nodata &  \nodata \nl
2201 &   41 &  4314.98 &   1.16 &  -1.13 &  mfw  &  \nodata &   21 &  \nodata &  \nodata &  \nodata &  150 &  183 &  183 &  \nodata &  \nodata \nl
2201 &   94 &  4316.81 &   2.05 &  -1.42 &  mfw  &  \nodata &  \nodata &   21 &  \nodata &  \nodata &   29 &   44 &   36 &   62 &  110 \nl
2201 &   41 &  4320.97 &   1.16 &  -1.87 &  mfw  &  \nodata &  \nodata &  \nodata &   62 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2201 &  104 &  4367.66 &   2.59 &  -1.27 &  mfw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   54 &   68 &   56 &  114 &  \nodata \nl
2201 &  104 &  4386.86 &   2.60 &  -1.26 &  mfw  &  \nodata &  \nodata &  \nodata &   35 &   58 &   47 &   70 &   52 &  103 &  114 \nl
2201 &   51 &  4394.06 &   1.22 &  -1.59 &  mfw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   54 &   88 &   78 &  155 &  \nodata \nl
2201 &   19 &  4395.03 &   1.08 &  -0.66 &  mfw  &   24 &   52 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2201 &   61 &  4395.85 &   1.24 &  -2.17 &  mfw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   58 &   65 &   71 &  \nodata &  \nodata \nl
2201 &   51 &  4399.77 &   1.24 &  -1.27 &  mfw  &  \nodata &   17 &  \nodata &   93 &  \nodata &  128 &  186 &  164 &  \nodata &  \nodata \nl
2201 &   51 &  4407.68 &   1.22 &  -2.47 & mfw   &  \nodata &  \nodata &  \nodata &  \nodata &   35 &   18 &  \nodata &  \nodata &  \nodata &   86 \nl
2201 &  115 &  4411.08 &   3.09 &  -1.06 & mfw   &  \nodata &  \nodata &  \nodata &   30 &   52 &   50 &   61 &   54 &   91 &   98 \nl
2201 &   40 &  4417.72 &   1.16 &  -1.43 & mfw   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  159 &  189 &  183 &  \nodata &  \nodata \nl
2201 &   93 &  4421.95 &   2.06 &  -1.77 & mfw   &  \nodata &  \nodata &  \nodata &  \nodata &   45 &   27 &   34 &   36 &   60 &  140 \nl
2201 &   40 &  4441.73 &   1.18 &  -2.41 & mfw   &  \nodata &  \nodata &  \nodata &   17 &  \nodata &   20 &   38 &   31 &   64 &  \nodata \nl
2201 &   19 &  4443.80 &   1.08 &  -0.70 & mfw   &  \nodata &   39 &  155 &  137 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2201 &   31 &  4444.56 &   1.12 &  -2.03 & mfw   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   33 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2201 &   19 &  4450.49 &   1.08 &  -1.45 & mfw   &  \nodata &   21 &   70 &   60 &  134 &   94 &  133 &  114 &  \nodata &  \nodata \nl
2201 &   40 &  4464.46 &   1.16 &  -2.08 & mfw   &  \nodata &  \nodata &   45 &   42 &   87 &   69 &   96 &   80 &  158 &  \nodata \nl
2201 &   31 &  4468.49 &   1.13 &  -0.60 & mfw   &  \nodata &   43 &  158 &  149 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2201 &   40 &  4470.86 &   1.16 &  -2.28 & mfw   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   29 &   55 &  \nodata &   93 &  135 \nl
2201 &  115 &  4488.32 &   3.12 &  -0.82 & mfw   &  \nodata &  \nodata &  \nodata &  \nodata &   71 &   55 &   75 &   74 &  117 &  \nodata \nl
2201 &   18 &  4493.53 &   1.08 &  -2.73 & mfw   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   40 \nl
2201 &   31 &  4501.27 &   1.12 &  -0.75 & mfw   &  \nodata &   36 &  121 &  \nodata &  \nodata &  192 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2201 &   18 &  4518.30 &   1.08 &  -2.56 & nk    &  \nodata &  \nodata &  \nodata &  \nodata &   40 &  \nodata &  \nodata &  \nodata &  \nodata &   90 \nl
2201 &   82 &  4529.47 &   1.57 &  -2.03 & nk    &  \nodata &  \nodata &  \nodata &   35 &   69 &   45 &   61 &   51 &   98 &  \nodata \nl
2201 &   60 &  4544.00 &   1.24 &  -2.40 &  mfw  &  \nodata &  \nodata &  \nodata &  \nodata &   17 &  \nodata &   18 &   20 &   42 &  \nodata \nl
2201 &   50 &  4563.76 &   1.22 &  -0.96 &  mfw  &   22 &   30 &  130 &  125 &  \nodata &  192 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2201 &   82 &  4571.97 &   1.57 &  -0.53 &  mfw  &  \nodata &   52 &  142 &  158 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2201 &   60 &  4580.46 &   1.23 &  -2.79 &  mfw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  104 \nl
2201 &   50 &  4589.96 &   1.24 &  -1.79 &  mfw  &  \nodata &  \nodata &   58 &   54 &  100 &   78 &  106 &   95 &  168 &  \nodata \nl
2201 &   49 &  4708.66 &   1.24 &  -2.21 &  mfw  &  \nodata &  \nodata &  \nodata &  \nodata &   44 &   19 &   27 &   20 &   52 &   83 \nl
2201 &   59 &  4719.52 &   1.24 &  -3.22 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   34 \nl
2201 &   92 &  4779.99 &   2.05 &  -1.37 &  mfw  &  \nodata &  \nodata &   40 &   35 &   83 &   51 &   77 &   75 &  124 &  160 \nl
2201 &   17 &  4798.54 &   1.08 &  -2.43 &  mfw  &  \nodata &  \nodata &  \nodata &  \nodata &   22 &  \nodata &  \nodata &  \nodata &  \nodata &   85 \nl
2201 &   92 &  4805.11 &   2.06 &  -1.10 &  mfw  &  \nodata &  \nodata &   55 &   65 &  113 &   97 &  122 &  116 &  188 &  \nodata \nl
2201 &  114 &  4874.03 &   3.09 &  -0.79 &  mfw  &  \nodata &  \nodata &  \nodata &   21 &  \nodata &   37 &   52 &   48 &   78 &  128 \nl
2201 &  114 &  4911.21 &   3.12 &  -0.34 &  mfw  &  \nodata &  \nodata &   59 &   38 &   66 &   60 &   78 &   69 &  109 &  127 \nl
2201 &  113 &  5010.20 &   3.10 &  -1.34 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   31 &   58 \nl
2201 &   71 &  5013.71 &   1.58 &  -1.94 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &   41 &  \nodata &   28 &  \nodata &   43 &   85 \nl
2201 &  113 &  5069.12 &   3.12 &  -1.39 &  mfw  &  \nodata &  \nodata &  \nodata &   13 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   67 \nl
2201 &  113 &  5072.30 &   3.12 &  -0.75 &  mfw  &  \nodata &  \nodata &  \nodata &   23 &   37 &  \nodata &  \nodata &   35 &   47 &   94 \nl
2201 &   86 &  5129.14 &   1.89 &  -1.39 &  mfw  &  \nodata &  \nodata &  \nodata &   27 &   76 &  852 &   81 &   69 &  105 &  130 \nl
2201 &   70 &  5154.06 &   1.57 &  -1.92 &  mfw  &  \nodata &  \nodata &   43 &   49 &   82 &   50 &   87 &  \nodata &  \nodata &  \nodata \nl
2201 &   86 &  5185.90 &   1.89 &  -1.35 &  mfw  &  \nodata &  \nodata &   47 &  \nodata &   70 &   44 &  \nodata &   56 &  106 &  130 \nl
2201 &   70 &  5188.70 &   1.58 &  -1.21 &  mfw  &  \nodata &   15 &   79 &   53 &  132 &  110 &  125 &  122 &  \nodata &  \nodata \nl
2201 &  103 &  5211.54 &   2.59 &  -1.36 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &   30 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2201 &   70 &  5226.53 &   1.57 &  -1.30 &  mfw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   67 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2301 &   32 &  4023.39 &   1.80 &  -0.52 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &   57 &  \nodata &  \nodata &  \nodata &   86 &  \nodata \nl
2400 &   22 &  4371.28 &   1.00 &  -1.09 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   42 \nl
2400 &    7 &  5204.52 &   0.94 &  -0.21 &  mfw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   33 &   86 \nl
2400 &    7 &  5206.04 &   0.94 &   0.02 &  mfw  &  \nodata &  \nodata &  \nodata &  \nodata &   41 &  \nodata &  \nodata &  \nodata &   34 &  150 \nl
2400 &    7 &  5208.40 &   0.94 &   0.16 &  mfw  &  \nodata &  \nodata &  \nodata &  \nodata &   42 &  \nodata &  \nodata &  \nodata &   53 &  130 \nl
2401 &  162 &  4145.77 &   5.32 &  -1.16 & nk   &  \nodata &  \nodata &  \nodata &   37 &  \nodata &  \nodata &   29 &  \nodata &   42 &   51 \nl
2401 &  162 &  4224.85 &   5.33 &  -1.06 & nk   &  \nodata &  \nodata &  \nodata &   48 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2401 &   31 &  4242.38 &   3.87 &  -1.17 & sl   &   24 &   38 &   74 &  108 &  \nodata &   92 &  117 &  110 &  164 &  155 \nl
2401 &   31 &  4252.62 &   3.86 &  -1.86 & sl   &  \nodata &   15 &  \nodata &  \nodata &  \nodata &  \nodata &   35 &   31 &  \nodata &  100 \nl
2401 &   31 &  4261.92 &   3.86 &  -1.34 & sl   &   31 &   31 &   50 &   75 &   82 &   79 &   92 &   85 &  132 &  140 \nl
2401 &   31 &  4269.28 &   3.85 &  -2.02 & sl   &  \nodata &    8 &  \nodata &  \nodata &  \nodata &   27 &   35 &   33 &   49 &   87 \nl
2401 &   31 &  4275.57 &   3.86 &  -1.47 & sl   &  \nodata &   18 &  \nodata &   57 &  \nodata &   64 &   58 &   63 &   82 &  \nodata \nl
2401 &   31 &  4284.21 &   3.85 &  -1.70 & sl   &  \nodata &   18 &   49 &   52 &   55 &   43 &   50 &   47 &   78 &  \nodata \nl
2401 &   39 &  4539.62 &   4.04 &  -2.53 & mfw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   37 \nl
2401 &   44 &  4555.02 &   4.07 &  -1.38 & mfw  &   21 &   28 &  \nodata &  \nodata &  \nodata &  66  &   83 &   82 &  121 &  \nodata \nl
2401 &   44 &  4558.66 &   4.07 &  -0.66 & mfw  &   68 &   79 &  123 &  \nodata &  \nodata &  189 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2401 &   39 &  4565.78 &   4.04 &  -2.11 & mfw  &  \nodata &  \nodata &  \nodata &   33 &   33 &  \nodata &   38 &   28 &   50 &   83 \nl
2401 &   44 &  4588.22 &   4.07 &  -0.63 & mfw  &   49 &   68 &  109 &  179 &  151 &  152 &  174 &  177 &  \nodata &  \nodata \nl
2401 &   44 &  4592.09 &   4.07 &  -1.22 & mfw  &  \nodata &   25 &   56 &   70 &   79 &  63  &   84 &   80 &  100 &  125 \nl
2401 &   44 &  4616.64 &   4.07 &  -1.36 & mfw  &  \nodata &   18 &   54 &   70 &   60 &   59 &   75 &   55 &  102 &  116 \nl
2401 &   44 &  4618.83 &   4.07 &  -0.84 & mfw  &   35 &   46 &   84 &  125 &  127 &  118 &  150 &  132 &  189 &  \nodata \nl
2401 &   44 &  4634.11 &   4.07 &  -0.96 & mfw  &  \nodata &   35 &  \nodata &  \nodata &   89 &   92 &  116 &  108 &  158 &  142 \nl
2401 &  177 &  4697.62 &   5.67 &  -1.62 & mfw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   28 \nl
2401 &   30 &  4812.35 &   3.86 &  -1.80 & mfw  &  \nodata &  \nodata &   21 &   31 &   36 &  24  &   35 &   24 &   40 &   62 \nl
2401 &   30 &  4824.12 &   3.87 &  -1.22 & mfw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  139 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2401 &   30 &  4824.13 &   3.87 &  -1.22 & mfw  &   42 &   53 &   95 &  138 &  133 &  \nodata &  155 &  156 &  \nodata &  \nodata \nl
2401 &   30 &  4836.22 &   3.86 &  -2.25 & mfw  &  \nodata &   15 &  \nodata &  \nodata &   41 &   27 &   41 &  \nodata &   58 &   77 \nl
2401 &   30 &  4848.24 &   3.86 &  -1.14 & mfw  &   31 &   45 &   81 &  115 &  118 &  \nodata &  148 &  134 &  179 &  \nodata \nl
2401 &   30 &  4858.24 &   3.86 &  -1.14 & mfw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  103 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2401 &   30 &  4876.41 &   3.86 &  -1.46 & mfw  &  \nodata &  \nodata &   65 &   89 &  100 &   88 &  110 &  110 &  145 &  \nodata \nl
2401 &   30 &  4884.58 &   3.86 &  -2.08 & mfw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   18 &  \nodata &  \nodata &  36 &  \nodata \nl
2501 &    5 &  4755.73 &   5.40 &  -1.24 & nk   &  \nodata &  \nodata &  \nodata &   25 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2600 &    4 &  3922.91 &   0.05 &  -1.65 &  fmw  &  \nodata &  \nodata &  \nodata &  \nodata &   73 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2600 &  278 &  4021.87 &   2.76 &  -0.77 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   78 \nl
2600 &   43 &  4045.82 &   1.48 &   0.28 &  ob   &  \nodata &   27 &   86 &   70 &  \nodata &  111 &  153 &  132 &  183 &  \nodata \nl
2600 &   43 &  4063.60 &   1.56 &   0.06 &  ob   &  \nodata &   22 &   75 &   57 &  116 &   77 &  115 &   84 &  151 &  \nodata \nl
2600 &   43 &  4071.74 &   1.61 &  -0.02 &  fmw  &  \nodata &  \nodata &   58 &   44 &   95 &   60 &   87 &   83 &  118 &  \nodata \nl
2600 &   43 &  4132.06 &   1.61 &  -0.67 &  ob   &  \nodata &  \nodata &  \nodata &   27 &  \nodata &   26 &   50 &  \nodata &  106 &  \nodata \nl
2600 &   43 &  4143.87 &   1.56 &  -0.51 &  ob   &  \nodata &  \nodata &   46 &  \nodata &  106 &  \nodata &   60 &   51 &  \nodata &  \nodata \nl
2600 &   42 &  4147.67 &   1.49 &  -2.10 &  fmw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   58 \nl
2600 &  354 &  4181.76 &   2.83 &  -0.32 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &   35 &  \nodata &  \nodata &  \nodata &  \nodata &  114 \nl
2600 &  152 &  4187.80 &   2.43 &  -0.61 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &   34 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2600 &  152 &  4198.31 &   2.40 &  -0.72 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   20 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2600 &  522 &  4199.10 &   3.05 &   0.14 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &   50 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2600 &   42 &  4202.03 &   1.48 &  -0.71 &  fmw  &  \nodata &  \nodata &   37 &  \nodata &   79 &   46 &   67 &   65 &  118 &  \nodata \nl
2600 &  152 &  4210.35 &   2.48 &  -0.87 &  fmw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   74 \nl
2600 &  693 &  4217.55 &   3.43 &  -0.48 &  ob   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   56 \nl
2600 &  152 &  4222.22 &   2.45 &  -0.97 &  fmw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   85 \nl
2600 &  152 &  4235.94 &   2.43 &  -0.32 &  ob   &  \nodata &  \nodata &  \nodata &  \nodata &   53 &   27 &   39 &   37 &   57 &  158 \nl
2600 &  693 &  4238.82 &   3.40 &  -0.23 &  ob   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   78 \nl
2600 &  152 &  4250.13 &   2.47 &  -0.38 &  ob   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   30 &   29 &  \nodata &  \nodata \nl
2600 &   42 &  4250.79 &   1.56 &  -0.71 & fmw   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   32 &   37 &  \nodata &  \nodata \nl
2600 &  152 &  4260.48 &   2.40 &   0.08 & ob    &  \nodata &  \nodata &   35 &   30 &   85 &   44 &   60 &   53 &   79 &  \nodata \nl
2600 &   42 &  4271.76 &   1.48 &  -0.17 & ob    &  \nodata &   10 &  \nodata &   54 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2600 &   71 &  4282.41 &   2.18 &  -0.78 & ob    &  \nodata &  \nodata &  \nodata &  \nodata &   48 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2600 &   42 &  4325.77 &   1.61 &   0.01 & ob    &  \nodata &   20 &  \nodata &  \nodata &  \nodata &   85 &  120 &   99 &  153 &  \nodata \nl
2600 &   41 &  4383.55 &   1.48 &   0.21 & ob    &  \nodata &   24 &  \nodata &  \nodata &  145 &  102 &  149 &  115 &  191 &  \nodata \nl
2600 &   41 &  4404.75 &   1.56 &  -0.15 & ob    &  \nodata &  \nodata &  \nodata &   39 &  119 &   65 &   91 &   82 &  128 &  \nodata \nl
2600 &    2 &  4427.31 &   0.05 &  -2.91 & fmwy  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   90 \nl
2600 &   68 &  4447.72 &   2.22 &  -1.34 & fmw   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   60 \nl
2600 &   68 &  4459.12 &   2.18 &  -1.33 & ob    &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   83 \nl
2600 &  350 &  4466.55 &   2.83 &  -0.59 & fmw   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   68 \nl
2600 &  350 &  4476.02 &   2.85 &  -0.82 & ob    &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   61 \nl
2600 &  828 &  4484.23 &   3.60 &  -0.86 & ob    &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   15 \nl
2600 &   68 &  4494.57 &   2.20 &  -1.14 & ob    &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  108 \nl
2600 &   68 &  4528.62 &   2.18 &  -0.89 & ob    &  \nodata &  \nodata &  \nodata &  \nodata &   58 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2600 &   39 &  4531.15 &   1.48 &  -2.10 & ob    &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   53 \nl
2600 &  554 &  4736.78 &   3.21 &  -0.75 & ob    &  \nodata &  \nodata &  \nodata &  \nodata &   28 &  \nodata &  \nodata &  \nodata &  \nodata &   65 \nl
2600 &  318 &  4890.76 &   2.88 &  -0.47 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   35 &  \nodata \nl
2600 &  318 &  4891.50 &   2.85 &  -0.17 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &   68 &  \nodata &  \nodata &  \nodata &   48 &  \nodata \nl
2600 &  318 &  4903.32 &   2.88 &  -1.08 &  fmw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   42 \nl
2600 &  318 &  4919.00 &   2.87 &  -0.34 &  fmw  &  \nodata &  \nodata &  \nodata &  \nodata &   34 &  \nodata &   32 &   21 &   45 &  112 \nl
2600 &  318 &  4920.51 &   2.83 &   0.07 &  fmw  &  \nodata &  \nodata &   34 &   23 &   68 &  \nodata &   61 &   39 &   77 &  \nodata \nl
2600 &  687 &  4966.10 &   3.33 &  -1.00 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   50 \nl
2600 &  114 &  5049.83 &   2.28 &  -1.42 &  fmw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   63 \nl
2600 & 1178 &  6024.07 &   4.55 &  -0.12 &  fmw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   55 \nl
2601 &    3 &  3914.48 &   1.67 &  -4.10 &  nk   &  \nodata &  \nodata &  \nodata &   88 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &    3 &  3930.31 &   1.70 &  -4.03 &  nk   &  \nodata &  \nodata &  \nodata &   88 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &  126 &  4032.95 &   4.50 &  -2.70 &  nk   &  \nodata &  \nodata &  \nodata &   32 &   42 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &  172 &  4048.83 &   5.57 &  -2.15 &  nk   &  \nodata &   14 &  \nodata &   45 &   50 &  \nodata &   46 &  \nodata &   48 &   86 \nl
2601 &  212 &  4057.51 &   7.27 &  -1.55 &  nk   &  \nodata &  \nodata &  \nodata &   20 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   28 &  4122.64 &   2.58 &  -3.38 &  nk   &  \nodata &   35 &   56 &   85 &   86 &   71 &   99 &   79 &  139 &  175 \nl
2601 &   22 &  4124.79 &   2.54 &  -4.20 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &   36 &  \nodata &   24 &   34 &  \nodata &   77 \nl
2601 &   27 &  4128.74 &   2.58 &  -3.77 &  fmw  &  \nodata &   14 &  \nodata &  \nodata &  \nodata &   60 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   27 &  4173.45 &   2.58 &  -2.18 &  fmw  &  \nodata &  \nodata &  130 &  \nodata &  \nodata &  183 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   28 &  4178.86 &   2.58 &  -2.48 &  fmw  &   78 &   81 &  \nodata &  \nodata &  \nodata &  188 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   28 &  4258.16 &   2.70 &  -3.40 &  fmw  &  \nodata &   24 &   63 &   66 &   93 &   65 &   86 &   80 &  141 &  \nodata \nl
2601 &   27 &  4273.32 &   2.70 &  -3.34 &  fmw  &  \nodata &   30 &  \nodata &   70 &   88 &   72 &   88 &   90 &  124 &  142 \nl
2601 &   32 &  4278.13 &   2.69 &  -3.82 &  nk   &  \nodata &   11 &  \nodata &   32 &  \nodata &  \nodata &   28 &  \nodata &   67 &  \nodata \nl
2601 &   28 &  4296.57 &   2.70 &  -3.01 &  fmw  &   59 &   55 &   78 &  132 &  125 &  121 &  141 &  141 &  \nodata &  \nodata \nl
2601 &   27 &  4303.17 &   2.70 &  -2.49 &  fmw  &   93 &   81 &  \nodata &  \nodata &  \nodata &  182 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   27 &  4351.76 &   2.70 &  -2.10 &  fmw  &  124 &   94 &  150 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &  213 &  4354.36 &   7.65 &  -1.34 &  nk   &  \nodata &  \nodata &  \nodata &   16 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   28 &  4369.40 &   2.78 &  -3.67 &  fmw  &  \nodata &  \nodata &  \nodata &   46 &   63 &   38 &   55 &   49 &   77 &  126 \nl
2601 &   27 &  4385.38 &   2.78 &  -2.57 &  fmw  &   75 &   70 &  \nodata &  170 &  \nodata &  165 &  189 &  183 &  \nodata &  \nodata \nl
2601 &   32 &  4413.60 &   2.68 &  -3.74 &  fmw* &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   54 \nl
2601 &   27 &  4416.82 &   2.78 &  -2.60 &  fmw  &   75 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   26 &  4461.43 &   2.58 &  -4.11 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  119 \nl
2601 &   37 &  4472.92 &   2.84 &  -3.43 &  fmw  &  \nodata &   22 &  \nodata &   52 &   55 &   49 &   58 &   47 &   84 &  108 \nl
2601 &   37 &  4489.19 &   2.83 &  -2.97 &  fmw  &   40 &   46 &  \nodata &  125 &  118 &  113 &  125 &  128 &  178 &  \nodata \nl
2601 &   37 &  4491.40 &   2.86 &  -2.70 &  fmw  &   50 &   59 &   95 &  142 &  135 &  134 &  155 &  153 &  \nodata &  \nodata \nl
2601 &   38 &  4508.28 &   2.86 &  -2.21 &  fmw  &  104 &   86 &  118 &  \nodata &  \nodata &  193 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   37 &  4515.34 &   2.84 &  -2.48 &  fmw  &   85 &   74 &  120 &  \nodata &  \nodata &  179 &  199 &  196 &  \nodata &  \nodata \nl
2601 &   37 &  4520.23 &   2.81 &  -2.60 &  fmw  &   68 &   70 &  108 &  178 &  152 &  160 &  191 &  188 &  \nodata &  \nodata \nl
2601 &   38 &  4522.63 &   2.84 &  -2.03 &  fmw  &  136 &  101 &  145 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   37 &  4534.17 &   2.86 &  -3.47 &  fmw  &   37 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   38 &  4541.52 &   2.86 &  -3.05 &  fmw  &   43 &   40 &   75 &  106 &  108 &   98 &  122 &  118 &  180 &  165 \nl
2601 &   37 &  4555.89 &   2.82 &  -2.29 &  fmw  &   96 &   81 &  \nodata &  \nodata &  \nodata &  193 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   38 &  4576.33 &   2.84 &  -2.82 &  nk   &   46 &   44 &   74 &  108 &  111 &   94 &  \nodata &  \nodata &  174 &  168 \nl
2601 &   37 &  4582.84 &   2.84 &  -3.10 &  fmw  &   28 &   36 &  \nodata &  \nodata &   98 &   81 &   87 &  103 &  141 &  \nodata \nl
2601 &   38 &  4583.83 &   2.81 &  -2.02 &  fmw  &  \nodata &  128 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   38 &  4620.51 &   2.83 &  -3.28 &  fmw  &  \nodata &   38 &   41 &   65 &   78 &   68 &   90 &   63 &  115 &  127 \nl
2601 &   37 &  4629.34 &   2.81 &  -2.37 &  fmw  &   91 &   82 &  130 &  \nodata &  \nodata &  189 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &  186 &  4635.33 &   5.96 &  -1.65 &  nk   &   41 &   30 &  \nodata &   55 &   37 &   43 &   48 &   41 &   70 &  \nodata \nl
2601 &   43 &  4656.97 &   2.89 &  -3.63 &  fmw  &  \nodata &   15 &  \nodata &   65 &   80 &   63 &   83 &   72 &  117 &  \nodata \nl
2601 &   44 &  4663.70 &   2.89 &  -4.26 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &   38 &   26 &   24 &  \nodata &   26 &   60 \nl
2601 &   37 &  4666.75 &   2.83 &  -3.33 &  fmw  &   21 &   27 &   51 &   68 &   70 &   62 &   80 &   60 &  115 &  135 \nl
2601 &   25 &  4670.17 &   2.58 &  -4.10 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   40 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   43 &  4731.44 &   2.89 &  -3.36 &  fmw  &   33 &   34 &   63 &   81 &   90 &   83 &  110 &   92 &  136 &  145 \nl
2601 &   36 &  4893.78 &   2.83 &  -4.45 &  fmw  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   34 \nl
2601 &   42 &  4923.92 &   2.89 &  -1.32 &  fmw  &  \nodata &  152 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   36 &  4993.36 &   2.81 &  -3.65 &  fmw  &  \nodata &  \nodata &   16 &  \nodata &   52 &  \nodata &   39 &   51 &   65 &   90 \nl
2601 &   42 &  5018.43 &   2.89 &  -1.22 &  fmw  &  \nodata &  154 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   35 &  5146.12 &   2.83 &  -3.91 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &   39 &  \nodata &  \nodata &  \nodata &  \nodata &   57 \nl
2601 &   35 &  5150.93 &   2.86 &  -4.45 & nk    &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   61 \nl
2601 &   42 &  5169.03 &   2.89 &  -0.87 & fmw   &  \nodata &  175 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   49 &  5197.57 &   3.23 &  -2.10 & fmw   &   87 &   76 &  112 &  \nodata &  \nodata &  164 &  \nodata &  194 &  \nodata &  \nodata \nl
2601 &   49 &  5234.62 &   3.22 &  -2.05 & fmw   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  171 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   46 &  5991.38 &   3.15 &  -3.59 & fmw*  &  \nodata &  \nodata &  \nodata &   12 &   41 &  \nodata &  \nodata &   31 &  \nodata &   88 \nl
2601 &  200 &  6103.54 &   6.22 &  -2.17 &  nk   &  \nodata &  \nodata &  \nodata &   25 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   74 &  6147.74 &   3.89 &  -2.46 & fmwy* &   22 &   37 &  \nodata &   57 &   80 &   62 &   65 &   69 &   78 &  100 \nl
2601 &   74 &  6149.24 &   3.89 &  -2.77 & fmw*  &   28 &   28 &  \nodata &   50 &   63 &   52 &   50 &   61 &   81 &   95 \nl
2601 &  200 &  6175.16 &   6.22 &  -1.98 & nk    &  \nodata &  \nodata &  \nodata &   25 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &  163 &  6179.38 &   5.57 &  -2.66 & fmw*  &  \nodata &  \nodata &  \nodata &   18 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   74 &  6238.38 &   3.89 &  -2.48 &  fmw* &  \nodata &  \nodata &  \nodata &   65 &  \nodata &  \nodata &   57 &  \nodata &  \nodata &  \nodata \nl
2601 &   74 &  6247.56 &   3.89 &  -2.36 &  fmw* &  \nodata &  \nodata &   70 &  115 &  \nodata &  113 &  129 &  114 &  161 &  159 \nl
2601 &  199 &  6331.97 &   6.22 &  -1.98 & nk    &  \nodata &  \nodata &  \nodata &   26 &   31 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   40 &  6416.08 &   2.89 &  -3.15 & fmw*  &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   65 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   74 &  6416.91 &   3.89 &  -2.55 &  fmw* &   49 &  \nodata &  \nodata &   45 &   60 &  53  &  \nodata &   64 &  \nodata &  116 \nl
2601 &   40 &  6432.65 &   2.89 &  -3.54 & fmw*  &  \nodata &  \nodata &  \nodata &  \nodata &   51 &   36 &  \nodata &   36 &  \nodata &  \nodata \nl
2601 &  199 &  6446.43 &   6.22 &  -2.01 & fmw*  &  \nodata &  \nodata &  \nodata &   30 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   74 &  6456.38 &   3.90 &  -2.15 & fmw*  &   77 &   70 &  \nodata &  150 &  \nodata &  142 &  \nodata &  \nodata &  \nodata &  \nodata \nl
2601 &   73 &  7307.97 &   3.89 &  -3.02 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   53 \nl
2601 &   73 &  7449.34 &   3.89 &  -3.31 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   27 &  \nodata &  \nodata &   29 &   72 \nl
2601 &   73 &  7462.38 &   3.89 &  -2.73 &  nk   &  \nodata &  \nodata &  \nodata &   35 &   90 &   37 &  \nodata &   66 &   63 &  110 \nl
3801 &    1 &  4077.71 &   0.00 &   0.15 & wm    &  \nodata &  \nodata &   58 &   43 &  110 &   59 &   98 &   81 &  175 &  \nodata \nl
3801 &    1 &  4215.52 &   0.00 &  -0.16 & wm    &  \nodata &  \nodata &   46 &   35 &  108 &   41 &   72 &   59 &  122 &  \nodata \nl
4001 &   54 &  4024.45 &   1.00 &  -0.97 &  nk   &  \nodata &   32 &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata \nl
4001 &   41 &  4149.22 &   0.80 &  -0.03 &  nk   &  \nodata &  \nodata &  \nodata &   17 &   46 &   27 &   36 &   43 &   68 &  138 \nl
4001 &   40 &  4496.96 &   0.71 &  -0.81 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &   49 \nl
5601 &    1 &  4934.09 &   0.00 &  -0.16 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &   53 &   19 &   23 &   13 &   54 &  196 \nl
5601 &    2 &  6496.90 &   0.60 &  -0.38 &  nk   &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  \nodata &  119 \nl
\tablecomments{
bghl = Bi\'emont \etal 1981,
mfw = Martin \etal 1988,
fmw = Fuhr \etal 1988,
fmwy = Fuhr \etal 1981,
ob = O'Brian \etal 1991,
op = Opacity Project (Hibbert \etal 1991), 
nk = new Kurucz (1990),
sl = Sigut \& Landstreet 1990,
wm = Wiese \& Martin 1980,
wsm = Wiese \etal 1969,
zhu = Zhu \etal 1989.
Some Fe II log(gf) values have been marked with a ``*''.   These have been
determined from analyses of the Sun, adopting log(Fe)+12=7.66.  This Fe 
value is 0.15~dex larger than the meteoritic abundance adopted here, and 
thus, those Fe II oscillator strengths have been raised by 0.15~dex.   }
\enddata
\end{deluxetable}


==> tab2.tex <==
%table 2
\begin{table*}
\caption[]{Atmospheric Parameter Uncertainties }
\begin{flushleft}
\begin{tabular} {lccc} 
\noalign{\smallskip}
\tableline
\noalign{\smallskip}
Star & \underline{ \ \ \ \ H$\gamma$ fits \ \ \ \ \ } & 
       \underline {Mg~I = Mg~II$\pm$0.2} & 
       \underline {\it \ LTE Mg $\pm$0.2 \ } \\
   & $\Delta$\teff \ \ \ $\Delta$\logg 
   & $\Delta$\teff \ \ \ $\Delta$\logg 
   & $\Delta$\teff \ \ \ $\Delta$\logg \\ 
\noalign{\smallskip}
\tableline
\noalign{\smallskip}
AV~110 & $\pm$200 \ \ \ $\pm$0.1 &  $\pm$250 \ \ \ $\pm$0.2 &  {\it +250 \ \ \ +0.2} \\
AV~298 & $\pm$200 \ \ \ $\pm$0.1 &  $\pm$200 \ \ \ $\pm$0.2 &  {\it +200 \ \ \ +0.1} \\
AV~392 & $\pm$200 \ \ \ $\pm$0.1 &  $\pm$200 \ \ \ $\pm$0.2 &  {\it +200 \ \ \ +0.1} \\
AV~136 & $\pm$100 \ \ \ $\pm$0.1 &  $\pm$100 \ \ \ $\pm$0.2 &  {\it +300 \ \ \ +0.1} \\ 
AV~463 & $\pm$100 \ \ \ $\pm$0.1 &  $\pm$100 \ \ \ $\pm$0.2 &  {\it +200 \ \ \ +0.2} \\ 
AV~478 & $\pm$100 \ \ \ $\pm$0.1 &  $\pm$150 \ \ \ $\pm$0.2 &  {\it +100 \ \ \ \phs0.0} \\ 
AV~254 & $\pm$100 \ \ \ $\pm$0.1 &  $\pm$150 \ \ \ $\pm$0.2 &  {\it +100 \ \ \ \phs0.0} \\ 
AV~442 & $\pm$100 \ \ \ $\pm$0.1 &  $\pm$150 \ \ \ $\pm$0.2 &  {\it +100 \ \ \ \phs0.0} \\ 
AV~213 & $\pm$100 \ \ \ $\pm$0.1 &  $\pm$100 \ \ \ $\pm$0.2 &  {\it +300 \ \ \ +0.2} \\ 
AV~174 & $\pm$200 \ \ \ $\pm$0.2 &  $\pm$250 \ \ \ $\pm$0.2 &  {\it +250 \ \ \ +0.2} \\ 
\noalign{\smallskip}
\tableline
\noalign{\smallskip}
\end{tabular}
\end{flushleft}
\end{table*}




==> tab3.tex <==
%table 3
\begin{deluxetable}{llllll} 
\tablewidth{0pc}
\tablecaption{ Elemental Abundances }
\tablehead{
\colhead{Elem} & \colhead{AV~110} & \colhead{AV~298} & \colhead{AV~392} & \colhead{AV~136}  & \colhead{AV~463} }
\startdata
C I      & $<$ 8.7            & $<$ 8.4            & $<$ 8.1 & $<$ 8.2            & $<$ 7.8            \nl
N I NLTE & 7.64 $\pm$0.18 (4) & 7.65 $\pm$0.21 (3) & $<$ 7.2 & 7.26 $\pm$0.07 (5) & 6.92 $\pm$0.25 (3) \nl
{\it \ N I LTE} & {\it 8.24 $\pm$0.23} & {\it 8.32 $\pm$0.23} & {\it $<$ 7.9} & 
                  {\it 8.18 $\pm$0.17} & {\it 7.50 $\pm$0.33} \nl 
O I NLTE  & 8.1               & 8.1                & 8.2        & 8.1                & 8.2  \nl 
{\it \ O I LTE} & {\it 8.4 $\pm$0.2 (S)} & {\it 8.4 $\pm$0.1 (S)} & {\it 8.4 (1)}
                & {\it 8.3 $\pm$0.2 (S)} & {\it 8.4 $\pm$0.2 (S)} \nl 
Na I  & \nodata             & \nodata             & 6.04           (1)  &  \nodata            & 5.57 $\pm$0.04 (2) \nl
Mg I NLTE & 6.87 (1)   & 7.03 $\pm$0.04 (3) & 6.83 $\pm$0.09 (4) & 6.77 $\pm$0.15 (4) & 6.99 $\pm$0.10 (3) \nl
{\it \ Mg I LTE}  & {\it 6.73} & {\it 6.91 $\pm$0.04} & {\it 6.81 $\pm$0.07} & 
                  {\it 6.74 $\pm$0.27} & {\it 6.89 $\pm$0.06} \nl
Mg II NLTE & 6.80 $\pm$0.01 (2) & 6.97 $\pm$0.18 (2) & 6.83 (1) & 6.82 $\pm$0.13 (3) & 7.02 $\pm$0.02 (3) \nl
{\it \ Mg II LTE} & {\it 6.89 $\pm$0.22} & {\it 7.16 $\pm$0.50} & {\it 7.19 } & 
                  {\it 6.97 $\pm$0.26} & {\it 7.07 $\pm$0.18} \nl
Si II & 7.21 $\pm$0.12 (3)  & 6.96 $\pm$0.29 (6)  & 7.26 $\pm$0.27 (3)  & 7.22 $\pm$0.08 (5)  & 6.86 $\pm$0.06 (3) \nl
Ca II & \nodata             & \nodata             & \nodata             & 5.46           (1)  & 5.56 $\pm$0.04 (2) \nl
Sc II & \nodata             & \nodata             & 2.42           (1)  & 2.28 $\pm$0.07 (2)  & 2.34 (1) \nl
Ti II & 4.04 $\pm$0.04 (3)  & 4.12 $\pm$0.10 (16) & 4.48 $\pm$0.16 (22) & 4.26 $\pm$0.12 (28) & 4.48 $\pm$0.17 (32) \nl
Cr I  & \nodata             & \nodata             & \nodata             & \nodata             & 5.21 $\pm$0.09 (2) \nl
Cr II & 4.78 $\pm$0.15 (8)  & 4.95 $\pm$0.18 (16) & 5.09 $\pm$0.16 (12) & 5.12 $\pm$0.20 (15) & 5.00 $\pm$0.19 (15) \nl
Fe I  & \nodata             & 6.67 $\pm$0.11 (5)  & 6.63 $\pm$0.15 (7)  & 6.54 $\pm$0.19 (9)  & 6.68 $\pm$0.18 (17) \nl
Fe II & 6.68 $\pm$0.21 (26) & 6.71 $\pm$0.16 (33) & 6.81 $\pm$0.16 (19) & 6.89 $\pm$0.15 (37) & 6.90 $\pm$0.18 (33) \nl
Sr II & \nodata             & \nodata             & 1.46 $\pm$0.10 (2)  & 1.32 $\pm$0.14 (2)  & 1.35 $\pm$0.19 (2) \nl
Zr II & \nodata             & \nodata             & \nodata             & 1.63           (1)  & 1.84  (1) \nl
Ba II & \nodata             & \nodata             & \nodata             & \nodata             & 1.56  (1) \nl
\enddata
\end{deluxetable}


==> tab4.tex <==
%table 3
\begin{deluxetable}{llllll} 
\tablewidth{0pc}
\tablecaption{ Elemental Abundance Uncertainties }
\tablehead{
\colhead{Elem} & \colhead{AV~110} & \colhead{AV~298} & \colhead{AV~392} & \colhead{AV~136}  & \colhead{AV~463} \\[.2ex]
               & \colhead{$\Delta$\teff= \ \ \ $\Delta$\logg} 
               & \colhead{$\Delta$\teff= \ \ \ $\Delta$\logg} 
               & \colhead{$\Delta$\teff= \ \ \ $\Delta$\logg} 
               & \colhead{$\Delta$\teff= \ \ \ $\Delta$\logg} 
               & \colhead{$\Delta$\teff= \ \ \ $\Delta$\logg} \\[.2ex]
               & \colhead{+200~K \ \ \ =$-$0.2} 
               & \colhead{+200~K \ \ \ =$-$0.2} 
               & \colhead{+200~K \ \ \ =$-$0.2} 
               & \colhead{+100~K \ \ \ =$-$0.2} 
               & \colhead{+100~K \ \ \ =$-$0.2} }
\startdata
N I & +0.06 \ \ \ +0.12 & +0.07 \ \ \ +0.11 & \phs\nodata \ \ \ \ \phs\nodata & 
          +0.04 \ \ \ +0.05 & +0.03 \ \ \ +0.04 \nl
O I & +0.06 \ \ \ +0.08 & +0.05 \ \ \ +0.06 & +0.04 \ \ \ +0.04 & 
         +0.02 \ \ \ +0.03 & +0.01 \ \ \ +0.03 \nl
Na I  &  \phs\nodata \ \ \ \ \phs\nodata & \phs\nodata \ \ \ \ \phs\nodata  & +0.20 \ \ \  +0.12 & \phs\nodata \ \ \ \ \phs\nodata  & +0.14 \ \ \  +0.16 \nl 
Si II & $-$0.02 \ \ \  $-$0.02 & $-$0.02 \ \ \ $-$0.02 & $-$0.02 \ \ \ $-$0.04 & $-$0.02 \ \ \  +0.03 & $-$0.02 \ \ \  +0.02 \nl
Mg I  & +0.20 \ \ \  +0.20 & +0.20 \ \ \  +0.19 & +0.24 \ \ \  +0.12 & +0.18 \ \ \  +0.18 & +0.14 \ \ \  +0.18 \nl
Mg II &  +0.01 \ \ \ +0.01 & \phs0.00 \ \ \ +0.01 & \phs0.00 \ \ \ \phs0.00 & \phs0.00 \ \ \  +0.01 & \phs0.00 \ \ \  +0.01 \nl
Ca II & \phs\nodata \ \ \ \ \phs\nodata & \phs\nodata \ \ \ \ \phs\nodata & \phs\nodata \ \ \ \ \phs\nodata  & +0.29 \ \ \  +0.14 & +0.18 \ \ \  +0.14 \nl
Sc II & \phs\nodata \ \ \ \ \phs\nodata & \phs\nodata \ \ \ \ \phs\nodata & +0.22 \ \ \  +0.05 & +0.16 \ \ \  +0.10 & +0.12 \ \ \  +0.09 \nl
Ti II & +0.16 \ \ \  +0.08 & +0.16 \ \ \ +0.08 & +0.16 \ \ \  +0.02 & +0.12 \ \ \  +0.06 & +0.09 \ \ \  +0.05 \nl
Cr II & +0.06 \ \ \ +0.02 & +0.07 \ \ \ \phs0.00 & +0.08 \ \ \ \phs0.00 & +0.07 \ \ \  +0.02 & +0.06 \ \ \  +0.02 \nl
Fe I  & \phs\nodata \ \ \ \ \phs\nodata & +0.17 \ \ \ +0.14 & +0.26 \ \ \  +0.12 & +0.22 \ \ \  +0.18 & +0.14 \ \ \  +0.18 \nl
Fe II & +0.04 \ \ \ \phs0.00 & +0.05 \ \ \ $-$0.02 & +0.10 \ \ \ \phs0.00 & +0.06 \ \ \  +0.01 & +0.06 \ \ \  +0.01 \nl
Sr II & \phs\nodata \ \ \ \ \phs\nodata & \phs\nodata \ \ \ \ \phs\nodata  & +0.30 \ \ \  +0.10 & +0.23 \ \ \  +0.18 & +0.17 \ \ \  +0.16 \nl
Zr II & \phs\nodata \ \ \ \ \phs\nodata & \phs\nodata \ \ \ \ \phs\nodata & \phs\nodata \ \ \ \ \phs\nodata & +0.12 \ \ \  +0.06 & +0.09 \ \ \  +0.04 \nl
Ba II & \phs\nodata \ \ \ \ \phs\nodata & \phs\nodata \ \ \ \ \phs\nodata & \phs\nodata \ \ \ \ \phs\nodata &  \phs\nodata \ \ \ \ \phs\nodata  & +0.18 \ \ \  +0.18 \nl
\enddata
\end{deluxetable}


==> tab5.tex <==
%table 3
\begin{deluxetable}{llllll} 
\tablewidth{0pc}
\tablecaption{ Elemental Abundances }
\tablehead{
\colhead{Elem} &  \colhead{AV~478} & \colhead{AV~254} &  \colhead{AV~442} &  \colhead{AV~213} & \colhead{AV~174} }
\startdata

C I  & $<$ 7.9 & $<$ 7.8 & $<$ 7.9 & $<$ 7.6 & $<$ 7.3 \nl
N I NLTE & 7.61 $\pm$0.16 (4) & 7.13 $\pm$0.27 (2) & 7.32 $\pm$0.21 (4) & 7.74 $\pm$0.22 (5) & 6.76  (1) \nl
{\it \ N I LTE} & {\it 8.43 $\pm$0.24} & {\it 7.84 $\pm$0.36} & {\it 8.07 $\pm$0.26} & 
                  {\it 8.36 $\pm$0.30} & {\it 7.07 } \nl
O I NLTE  & 8.1  & 8.2 & 8.2  & 8.0 & 8.2 \nl
{\it O I LTE} & {\it 8.3 $\pm$0.1 (S)} & {\it 8.4 $\pm$0.1 (S)} & {\it 8.4 $\pm$0.1 (4)} 
              & {\it 8.1 $\pm$0.1 (S)} & {\it 8.3 $\pm$0.2 (S)} \nl
Na I  & 5.86 $\pm$0.21 (3)  & 6.00  (1)  & 5.82  (1)  & \nodata  & 5.55 (1) \nl
Mg I NLTE & 6.76 $\pm$0.07 (4) & 6.79 $\pm$0.08 (3) & 6.72 $\pm$0.11 (3) & 6.78 $\pm$0.05 (2) & 6.69 (1) \nl
{\it \ Mg I LTE} & {\it 6.70 $\pm$0.08} & {\it 6.71 $\pm$0.06} & {\it 6.62 $\pm$0.10} & 
                      {\it 6.66 $\pm$0.05} & {\it 6.65} \nl 
Mg II NLTE & 6.83 $\pm$0.07 (4) & 6.84 $\pm$0.13 (4) & 6.71 $\pm$0.03 (3) & 6.77 $\pm$0.10 (2) & 6.74 (1) \nl
{\it \ Mg II LTE} & {\it 6.90 $\pm$0.16} & {\it 6.89 $\pm$0.04} & {\it 6.73 $\pm$0.20} & 
                          {\it 6.86 $\pm$0.01} & {\it 6.97} \nl
Si II & 6.88 $\pm$0.13 (4)  & 6.79 $\pm$0.12 (4)  & 6.71 $\pm$0.06 (5)  & 6.94 $\pm$0.14 (4)  & 6.91 $\pm$0.16 (2) \nl
Ca I  & 5.26 (1) & 5.31 (1)            & 5.26 (1)            & 5.20 (1)            & 5.97 $\pm$0.15 (5) \nl
Ca II & \nodata & 5.31 $\pm$0.25 (2)  & 5.21 $\pm$0.05 (2)  & 5.40 $\pm$0.35 (2)  & 5.38  (1) \nl
Sc II & 2.12 $\pm$0.27 (4)  & 2.28 $\pm$0.07 (3)  & 2.22 $\pm$0.15 (4)  & 2.22 $\pm$0.19 (3)  & 2.27 $\pm$0.18 (3) \nl 
Ti II & 4.33 $\pm$0.19 (35) & 4.39 $\pm$0.20 (35) & 4.28 $\pm$0.19 (35) & 4.25 $\pm$0.22 (28) & 4.31 $\pm$0.26 (21) \nl
Cr I  & \nodata             & \nodata             & \nodata             & 5.04 $\pm$0.11 (3)  & 5.25 $\pm$0.26 (4) \nl
Cr II & 4.93 $\pm$0.13 (17) & 4.99 $\pm$0.16 (18) & 4.87 $\pm$0.18 (17) & 4.90 $\pm$0.18 (15) & 5.06 $\pm$0.23 (13) \nl
Fe I  & 6.46 $\pm$0.17 (10) & 6.58 $\pm$0.19 (15) & 6.52 $\pm$0.22 (15) & 6.61 $\pm$0.22 (23) & 6.89 $\pm$0.17 (22) \nl
Fe II & 6.80 $\pm$0.16 (31) & 6.80 $\pm$0.16 (31) & 6.71 $\pm$0.14 (30) & 6.71 $\pm$0.16 (24) & 6.86 $\pm$0.23 (25) \nl
Sr II & 1.09 $\pm$0.07 (2)  & 1.20 $\pm$0.07 (2)  & 1.07 $\pm$0.08 (2)  & 1.00 (1)  & \nodata \nl
Zr II & 1.65 (1)  & 1.72 (1)  & 1.75 (1)  & 1.62 (1)  & 1.94 $\pm$0.10 (2) \nl
Ba II & 1.40 (1)  & 1.31 (1)  & 1.24 (1)  & 1.34 $\pm$0.25 (2)  & 1.66  (1) \nl
\enddata
\end{deluxetable}


==> tab6.tex <==
%table 3
\begin{deluxetable}{llllll} 
\tablewidth{0pc}
\tablecaption{ Elemental Abundance Uncertainties }
\tablehead{
\colhead{Elem} & \colhead{AV~478} & \colhead{AV~254} & \colhead{AV~442} & \colhead{AV~213}  & \colhead{AV~174} \\[.2ex]
               & \colhead{$\Delta$\teff= \ \ \ $\Delta$\logg} 
               & \colhead{$\Delta$\teff= \ \ \ $\Delta$\logg} 
               & \colhead{$\Delta$\teff= \ \ \ $\Delta$\logg} 
               & \colhead{$\Delta$\teff= \ \ \ $\Delta$\logg} 
               & \colhead{$\Delta$\teff= \ \ \ $\Delta$\logg} \\[.2ex]
               & \colhead{+150~K \ \ \ =$-$0.2} 
               & \colhead{+150~K \ \ \ =$-$0.2} 
               & \colhead{+150~K \ \ \ =$-$0.2} 
               & \colhead{+100~K \ \ \ =$-$0.2} 
               & \colhead{+200~K \ \ \ =$-$0.2} }
\startdata
N I  & +0.08 \ \ \ +0.04 & +0.06 \ \ \ +0.06 & +0.07 \ \ \ +0.10 & 
         +0.04 \ \ \ +0.06 & +0.01 \ \ \ +0.02 \nl
O I   & +0.05  \ \ \ +0.02 & +0.04 \ \ \ +0.05 & +0.06 \ \ \ +0.08 & 
        +0.03 \ \ \ +0.04 & +0.06 \ \ \ +0.04 \nl
Na I  & +0.26 \ \ \  +0.17 & +0.26 \ \ \ +0.21 & +0.30 \ \ \ +0.28 & +0.19 \ \ \ +0.25 & +0.22 \ \ \ +0.13 \nl
Mg I  & +0.26 \ \ \  +0.18 & +0.26 \ \ \ +0.21 & +0.29 \ \ \ +0.30 & +0.20 \ \ \ +0.25 & +0.23 \ \ \ +0.14 \nl
Mg II & \phs0.00 \ \ \ \phs0.00 & +0.02 \ \ \ +0.03 & +0.02 \ \ \ +0.02 & +0.02 \ \ \ +0.03 & \phs0.00 \ \ \ \phs0.00 \nl
Si II & $-$0.02 \ \ \ $-$0.02 & $-$0.02 \ \ \ $-$0.01 & $-$0.03 \ \ \ \phs0.00 & +0.01 \ \ \ +0.04 & $-$0.01 \ \ \ $-$0.01 \nl
Ca II & +0.22 \ \ \ +0.13 & +0.19 \ \ \ +0.17 & +0.22 \ \ \ +0.28 & +0.16 \ \ \ +0.20 & +0.12 \ \ \ +0.08 \nl
Sc II & +0.24 \ \ \ +0.08 & +0.23 \ \ \ +0.12 & +0.27 \ \ \ +0.18 & +0.17 \ \ \ +0.13 & +0.19 \ \ \ +0.04 \nl
Ti II & +0.19 \ \ \ +0.05 & +0.17 \ \ \ +0.08 & +0.19 \ \ \ +0.14 & +0.13 \ \ \ +0.10 & +0.16 \ \ \ +0.02 \nl
Cr II & +0.11 \ \ \ +0.02 & +0.11 \ \ \ +0.04 & +0.14 \ \ \ +0.08 & +0.09 \ \ \ +0.08 & +0.11 \ \ \ +0.02 \nl
Fe I  & +0.29 \ \ \ +0.18 & +0.29 \ \ \ +0.22 & +0.32 \ \ \ +0.30 & +0.26 \ \ \ +0.26 & +0.27 \ \ \ +0.14 \nl
Fe II & +0.11 \ \ \ +0.02 & +0.11 \ \ \ +0.04 & +0.12 \ \ \ +0.08 & +0.09 \ \ \ +0.07 & +0.13 \ \ \ +0.01 \nl
Sr II & +0.34 \ \ \ +0.16 & +0.33 \ \ \ +0.21 & +0.37 \ \ \ +0.30 & +0.26 \ \ \ +0.25 & \phs\nodata \ \ \ \ \phs\nodata \nl
Zr II & +0.18 \ \ \ +0.04 & +0.17 \ \ \ +0.07 & +0.29 \ \ \ +0.14 & +0.15 \ \ \ +0.11 & +0.18 \ \ \ +0.03 \nl
Ba II & +0.35 \ \ \ +0.17 & +0.34 \ \ \ +0.22 & +0.37 \ \ \ +0.32 & +0.27 \ \ \ +0.27 & +0.35 \ \ \ +0.13 \nl
\enddata
\end{deluxetable}


==> tab7.tex <==
%table 0
\begin{table*}
\caption[]{SMC and Galactic A-Type Supergiant Abundances (Relative to Solar)}
\begin{flushleft}
\begin{tabular}{lllll} 
\noalign{\smallskip}
\tableline
\noalign{\smallskip}
     & SUN &       SMC AIs           & SMC AIs & Galactic AIs \\
Elem &     &  AVER  $\pm\sigma$ (\#) & [M/H] & [M/H] (N)    \\
\noalign{\smallskip}
\tableline
\noalign{\smallskip}
N I   & 7.8$^a$ & 7.33 $\pm$0.35 ( 9) & $-$0.47$^a$ &   +0.25 (22) \\
O I   & 8.6$^a$ & 8.14 $\pm$0.10 ( 9) & $-$0.46$^a$ & $-$0.01$^b$ (22) \\
Na I  & 6.31 & 5.81 $\pm$0.22 ( 6) & $-$0.50 &   +0.66 (11) \\
Mg I  & 7.58 & 6.82 $\pm$0.11 (10) & $-$0.76 & $-$0.10 (19) \\
Mg II & 7.58 & 6.83 $\pm$0.10 (10) & $-$0.75 & $-$0.12 (22) \\
Si II & 7.55 & 6.97 $\pm$0.18 (10) & $-$0.58 & $-$0.22 ( 5) \\
Ca I  & 6.34 & 5.23 $\pm$0.14 ( 4) & $-$1.11 &   +0.31 (15) \\
Ca II & 6.34 & 5.39 $\pm$0.16 ( 6) & $-$0.95 & $-$0.31 (10) \\
Sc II & 3.09 & 2.28 $\pm$0.17 ( 8) & $-$0.81 &   +0.04 ( 9) \\
Ti II & 4.93 & 4.29 $\pm$0.15 (10) & $-$0.64 & $-$0.07 (22) \\
Cr I  & 5.68 & 5.17 $\pm$0.15 ( 3) & $-$0.51 &   +0.21 ( 8) \\
Cr II & 5.68 & 4.97 $\pm$0.11 (10) & $-$0.71 & $-$0.07 (18) \\
Fe I  & 7.51 & 6.62 $\pm$0.15 ( 9) & $-$0.89 &   +0.05 (22) \\
Fe II & 7.51 & 6.78 $\pm$0.07 (10) & $-$0.73 & $-$0.11 (22) \\
Sr II & 2.93 & 1.21 $\pm$0.19 ( 7) & $-$1.72 & $-$0.52 ( 4) \\
Zr II & 2.61 & 1.74 $\pm$0.13 ( 7) & $-$0.87 &   +0.20 ( 3) \\
Ba II & 2.21 & 1.42 $\pm$0.19 ( 6) & $-$0.79 &  \nodata   \\
\noalign{\smallskip}
\tableline
\noalign{\smallskip}
\end{tabular} 
\begin{minipage}[t]{18cm}{
$^a$Note that solar neighbourhood abundances are adopted for 
these elements (discussed in Section 6.1, also see Table 9).

$^b$The same NLTE corrections applied to the SMC O~I abundances
have been applied here to the Galactic A-supergiant LTE abundances
from Venn (1995a).}
\end{minipage}

\end{flushleft}
\end{table*}



==> tab8.tex <==
%table 7
\begin{table*}
\caption[]{Differential (``like $-$ like'') Abundances for SMC Stars}
\begin{flushleft}
\begin{tabular}{llrrrrrrr} 
\noalign{\smallskip}
\tableline
\noalign{\smallskip}
     & Solar  & A~Is$^a$ & LL92$^b$ & RB89$^c$ & S89$^c$ & H97$^{d,g}$ & L98$^e$ &  BIIIs$^f$ \\
Elem & Neigh. & ($\le$10 stars) & ($\le$7 stars) & ($\le$8 stars) & ($\le$3 stars) & ($\le$6 stars) & ($\le$6 stars) & ($\le$6 stars)\\
\noalign{\smallskip}
\tableline
\noalign{\smallskip}
C     & 8.3 & ...    & $-$0.6     & $-$0.5 & $-$0.7 & $-$0.8 & $-$0.7 & $<-$0.4 \\
N     & 7.8 & $-$0.8 & $-$0.9     &    ... &   ...  & $-$0.3 & ...    & $>-$0.9 \\
O     & 8.6 & $-$0.5 & $-$0.4     &    ... & $-$0.6 & $-$0.7 & $-$0.7 & $-$0.6 \\
Na    & 6.3 & $-$1.1 & $-$0.9     & $-$0.4 & $-$0.7 & $-$0.7 & $-$1.0 &  ... \\
Mg    & 7.6 & $-$0.7 & $-$0.5     & $-$0.6 & $-$0.7 & $-$0.5 & $-$0.8 & $-$0.6 \\
Si    & 7.6 & $-$0.3 & $-$0.4     &    ... & $-$0.5 & $-$0.8 & $-$0.8 & $-$0.9 \\
Ca    & 6.3 & $-$0.6 & $-$0.5     & $-$0.2 & $-$0.6 & $-$0.8 & $-$0.6 & ... \\
Sc    & 3.1 & $-$0.8 & $-$0.4$^g$ & $-$0.5 & $-$0.6 & $-$0.9 & $-$0.9 & ... \\
Ti    & 4.9 & $-$0.7 & $-$0.6     & $-$0.5 & $-$0.8 & $-$0.7 & $-$0.7 &    ... \\
Cr    & 5.7 & $-$0.6 & $-$0.4$^g$ & $-$0.4 & $-$0.6 & $-$1.0 & $-$0.7 &    ... \\
Fe I  & 7.5 & $-$0.9 & $-$0.6     & $-$0.5 & $-$0.6 & $-$0.7 & $-$0.7 & ...  \\
Fe II & 7.5 & $-$0.6 & $-$0.6     & $-$0.6 & $-$0.6 & $-$0.7 & $-$0.7 & ... \\
Sr    & 2.9 & $-$1.2 &    ...     & $-$1.4 &   ...  & ... & ...    & ... \\
Zr    & 2.6 & $-$1.0 &    ...     & $-$0.6 & $-$0.5 & ... & $-$0.9 & ... \\
Ba    & 2.2 & $-$0.8$^g$ & ...    & $-$0.9 & $-$0.6 & ... & ...    & ... \\
\noalign{\smallskip}
\tableline
\noalign{\smallskip}
\end{tabular} 
\begin{minipage}[t]{18cm}{

$^a$ A Is = SMC (this paper) minus Galactic (Venn 1995a,b) 
     A-supergiant abundances. 

$^b$ LL92 = SMC (Luck \& Lambert 1992) minus Galactic (Luck \& Lambert 1985) 
     F-K supergiant abundances.

$^c$ RB89, S89 = SMC F-G supergiants (Russell \& Bessell 1989, 
     Spite \etal 1989a,b) minus Canopus abundances.

$^d$ H97 = SMC K supergiant (Hill \etal 1997a,b) minus solar abundances

  \ \ (their comparison star, Arcturus, is metal-poor with [Fe/H]=$-$0.5).  

$^e$ L98 = SMC F-K supergiant and Cepheid (Luck \etal 1998) 
           minus Galactic F-K supergiant (Luck \etal 1998) abundances.

$^f$ BIIIs = mean of 6 differential B-giant abundances: 

\ \ \ \ (1) IDK-D2 minus 67 Oph (Rolleston \etal 1993),

\ \ \ \ (2) AV175, NGC330-B30, NGC330-B22 minus HR 2618
              (J\"uttner \etal 1992), 

\ \ \ \ (3) NGC330-B30 minus HR 3663 (Reitermann \etal 1991),

\ \ \ \ (4) NGC330-A01, NGC330-B04 (Lennon \etal 1996) relative to $\tau$ Sco
            
\ \ \ \  \ \ \  \ \ (from Rolleston \etal 1993).

$^g$ Abundances that are relative to the solar neighborhood (column 1)
and not the comparison stars. 
}
\end{minipage}
\end{flushleft}
\end{table*}


==> tab9.tex <==
%table 8
\begin{table*}
\caption[]{Galactic Nebular and B-Star Abundances}
\begin{flushleft}
\begin{tabular}{cc|llcllll|lcl|c} 
\noalign{\smallskip}
\tableline
\noalign{\smallskip}
Elem & SUN & & & Orion      & & & &  & &            B-stars  & & Adopted \\
     &     &  D84 & B91 & R91 & O92 & W92 & P93 & E98 &  GL  & K  & CL &  \\
     &     &  & & & & 0/0.055$^a$ & 0/0.04$^a$ & g/g+d$^b$  &    &    &  \\
\noalign{\smallskip}
\tableline
\noalign{\smallskip}
C &  8.6 & 8.2 & 8.3 & 8.5* & 8.6 & 7.9/8.8 & 8.5/8.5 & 8.4/8.5 & 8.2 & 8.2 & 8.4 & 8.3 \\
N &  8.0 & 7.5 & 7.9 & 7.8  & 7.6 & 7.5/7.7 & 7.7/7.9 & 7.8/7.8 & 7.8 & 7.8 & 7.8 & 7.8 \\
O &  8.9 & 8.7 & 8.6 & 8.6  & 8.5 & 8.4/8.9 & 8.5/8.8 & 8.6/8.7 & 8.7 & 8.6 & 8.6 & 8.6 \\
\noalign{\smallskip}
\tableline
\noalign{\smallskip}
\end{tabular} 
\begin{minipage}[t]{18cm}{

D84 = Dufour 1984, B91 = Baldwin \etal 1991, R91 = Rubin \etal 1991
(* Same C in Rubin et al 1993), O92 = Osterbrock \etal 1992, 
W92 = Walter \etal 1992, P93 = Peimbert \etal 1993, E98 = Esteban \etal 1998,
GL = Gies \& Lambert 1992, K = Kilian 1992, CL = Cunha \& Lambert 1994.
Solar abundances from Anders \& Grevesse 1989, Grevesse \& Noels 1993. 

$^a$ Different abundances depend on the estimated temperature
fluctuations as 0\%, 5.5\%, or 4\%. 

$^b$ Abundances from nebular gas measurements only (g), and those
corrected for dust depletions (g+d).
}
\end{minipage}
\end{flushleft}
\end{table*}


